An Empirical Study of Pre-trained Model Selection for Out-of-Distribution Generalization and Calibration

In the field of computer vision, fine-tuning pre-trained models has become a prevalent strategy for out-of-distribution (OOD) generalization tasks. Different from most prior work that has focused on advancing learning algorithms, we systematically examined how pre-trained model size, pre-training dataset size, and training strategies impact generalization and confidence calibration on downstream tasks. We evaluated 100 models across diverse pre-trained model sizes, five pre-training datasets, and five data augmentations through extensive experiments on four distribution shift datasets totaling over 120,000 GPU hours. Our results demonstrate the significant impact of pre-trained model selection, with optimal choices substantially improving OOD accuracy over algorithm improvement alone. Additionally, we find that larger models and bigger pre-training datasets not only enhance OOD performance but also improve calibration, helping to mitigate overconfidence, contrary to some prior studies that found modern deep networks to calibrate worse than classical shallow models. Our work underscores the overlooked importance of pre-trained model selection for out-of-distribution generalization and calibration.

==> section/body.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}[h]
    \vspace{-4mm}
    \centering
    \includegraphics[width=\linewidth]{figs/all-all-avg_test_acc-avg_test_ece-full2.pdf}
    \caption{This paper investigates the out-of-distribution (OOD) generalization and uncertainty calibration of a total of \update{100} ImageNet pre-trained models on \update{five} datasets from DomainBed~\citep{Gulrajani21} \update{and WILDS~\citep{koh2021wilds}}. These panels show the relationship between expected calibration error (ECE) rates (lower is better) and OOD test accuracy (higher is better). Marker sizes are proportional to the number of model parameters, and marker shapes correspond to pre-training configurations. We can observe a general trend that \textbf{larger models achieve the best of both worlds (bottom-right corner)}, except for \modelname{VGGs} and \modelname{MLP-Mixers}. The full legend can be found in \cref{ap:fig:all-all-test-acc-test-ece}.}
    \label{fig:all-test-acc-test-ece}
    \vspace{-4mm}
\end{figure}


\begin{table}[b]
    
% \begin{wraptable}[4]{r}{8cm}
    % \resizebox{5cm}{!}{%
    \vspace{-4mm}
    \centering
    \begin{tabular}{lccMcc}
         \toprule
         & ERM       &   Best Alg.    &   Best Model   &  $\Delta$     \\
    \cmidrule(ll){1-1} \cmidrule(rl){2-4} \cmidrule(rr){5-5}
    PACS & 88.1                  &   89.1                            &   96.7     &  +7.71            \\
    OfficeHome & 62.7            &   64.7                            &   87.4     &  +22.7            \\
    DomainNet  & 58.4            &   59.5                            &   77.8     &  +18.3            \\
    VLCS & 76.4                  &   77.5                            &   82.2     &  +4.7            \\ 
        % \cmidrule(ll){1-1} \cmidrule(rl){2-4} \cmidrule(rr){5-5}
    % {Camelyon\footnotemark}&  96.8   & -          &     97.6   &              \\                  
    \bottomrule
    \end{tabular}
    \caption{
    Comparison of OOD test accuracy of \modelname{ResNet-50} trained with ERM~\citep{vapnik1991principles}, \modelname{ResNet-50} with the best algorithms (Best Alg.) reported in~\cite{Gulrajani21}, and a larger model (ViT-base pre-trained on ImageNet-21k for VLCS and ViT-large pre-trained on ImageNet-21k for other tasks) trained with ERM. $\Delta$ indicates the improvement from results with the best algorithms to results with the best models. Baseline results are adopted from~\cite{Gulrajani21}.
    }
    \label{tab:improvement}
    % \vspace{-3mm}
    % }
% \end{wraptable}
\end{table}


% \footnotetext{WILDSCamelyon datasets is introduced by \citet{bandi2018detection}}




% ================================== Structure of Introduction ==================================

% [Problem statement]: 
% Briefly introduce the problem of out-of-distribution (OOD) generalization and uncertainty calibration. Highlight their importance in developing robust AI systems.

% [Current approaches]: 
% Discuss the existing approaches to tackling these challenges, particularly focusing on the prevalent fine-tuning strategy.

% [Limitations of current approaches]: 
% Identify the limitations of current research, emphasizing the under-exploration of pre-trained model selection's impact.

% [Our contribution]: 
% Clearly state the novelty of this research and its contributions to the field.

% [Research question/hypotheses]: 
% Explicitly mention the research question or hypotheses investigated in the study.

% [Methodology]: 
% Briefly describe the methodology employed in the research, including the pre-trained models, datasets, and evaluation metrics.

% [Key findings]: 
% Summarize the key findings and their implications, highlighting the significance of the results.
% ================================== Structure of Introduction ==================================

% \rev{Green: modified part after yesterday's meeting}

% [General problem statement]: 
Out-of-distribution (OOD) generalization and uncertainty calibration have become critical challenges in recent years. This stems from their indispensable role in developing robust and reliable artificial intelligence across diverse tasks and situations~\citep{Nagarajan21, Geirhos20, shen2021towards, Zhou21}.
Our research holds particular relevance to practical contexts requiring OOD generalization and reliable inference in computer vision, such as domain generalization tasks~\citep{arjovsky2019invariant, ghifary2015domain, li2017deeper, fang2013unbiased, venkateswara2017deep, peng2019moment}, and uncertainty calibration tasks~\citep{naeini2015obtaining,guo2017calibration,krishnan2020improving} which aims to ensure that the estimated class probabilities are consistent with what would naturally occur. 
% [Current approaches]: 
Currently, the prevalent strategy for tackling these issues relies on fine-tuning---adjusting the parameters of pre-trained models to optimize performance on specified downstream tasks~\citep{Gulrajani21}. 

% [Limitations of current approaches 1 - predominant to focus on algorithm]: 
\update{
A limitation of current approaches is that existing research has predominantly focused on advancing learning algorithms~\citep{Arjovsky19, rame2022fishr, krueger2021out, sun2016deep, sagawa2019distributionally, yan2020improve,blanchard2021domain,koyama2020invariance, ahuja2021invariance}, with limited investigation into how the choice of pre-trained model affects OOD generalization and calibration. 
More recent studies~\citep{ li2022sparse, cha2022domain, arpit2022ensemble, zhang2023unified} have evaluated their proposed methodology on more modern architectures, like vision transformers;
however, they also used a limited number of pre-trained models solely to benchmark the effectiveness of their proposed OOD generalization algorithms.
While this approach has yielded significant progress, it often overlooks the crucial impact of pre-trained model selection on OOD generalization and calibration.
}

% [Limitations of current approaches 2 - no systematic work to reveal model size and dataset size effect]: 
\update{
Recently, some work ~\citet{ goldblum2023battle, vishniakov2023convnet, zhang2022delving} 
has studied the effects of pre-trained model selection on OOD generalization; however, it has used a limited variety in sizes and types of architectures of the pre-trained models. 
Those studies' scope was insufficient to reveal some of the trends we demonstrate in the present paper. 
}
\rev{
\citet{goldblum2023battle} evaluates several model architectures and model sizes as backbones in various downstream tasks but does not evaluate ECE in OOD, nor does it evaluate the scaling laws in model size and dataset size that we found. Instead, they focus on providing practitioners with a ranking of which model architecture best suits each task. \citet{zhang2022delving} focuses on evaluating \modelname{Vision Trainformer (ViT)} models only, while \citet{vishniakov2023convnet} focuses on both \modelname{ViT} and \modelname{ConvNext} models. These two studies involve a multifaceted evaluation of the models, including OOD generalization and calibration.
}
\rev{
Furthermore, a calibration study by \citep{minderer2021revisiting} noted that ECE worsens with larger models, especially when trained from scratch. Our work diverges significantly from these studies by examining pre-trained models across a broad spectrum of architectures, training strategies, sizes, and datasets. We specifically focus on how the parameters of pre-trained models and the size of pre-training datasets influence OOD generalization and calibration, aspects previously not fully explored.
}
\rev{
In \cref{sec:relatedworks}, we provide more details on the related work.
}

% [Our contribution]: 
\update{
Motivated by these limitations, we conduct a comprehensive and systematic evaluation of pre-trained model selection for OOD generalization and calibration.
We have found that pre-trained model selection is more powerful than initially thought, leading to substantial performance improvements over algorithmic enhancements (See \cref{tab:improvement}).
}

% [Methodology]:  Position of Our Work
We evaluate pre-trained models along three dimensions: (1) pre-trained model parameter size and architecture, (2) pre-training dataset size, (3) model design and training strategy for pre-trained models. We assess performance on downstream tasks using two key metrics: accuracy and expected calibration error (ECE)~\citep{naeini2015obtaining} under distributional shift.
\rev{
The few existing studies for this setting do not thoroughly explore all three axes above,
an exploration that is important for achieving the best results from model selection and for investigating this factor.
}

Through extensive experiments on five distribution shift datasets, we provide new insights into pre-trained model selection for OOD generalization and calibration in computer vision.
% [Methodology]:  What do we do, and what results?
Specifically, we evaluated 100 pre-trained models, spanning five pre-training datasets (ImageNet-1k to 22k and JFT-300M \citep{sun2017revisiting}), five data augmentation strategies, and several pre-training algorithms (including DINO \citep{caron2021emerging}, MAE \citep{he2022masked}, AdvProp \citep{xie2020adversarial}, Noisy Student \citep{xie2020self}) \update{and CLIP \citep{clip_paper}} on downstream tasks over five distribution shift datasets. 
Our extensive experiments, involving over \update{120,000} GPU hours, consistently show that larger models and more extensive datasets improve OOD generalization and calibration.
As can be seen in \cref{tab:improvement}, compared to learning algorithm improvements (up to 2\% on DomainBed~\citep{Gulrajani21}), the best pre-trained model selection boosts OOD accuracy dramatically (up to 22.7\% in our experiments). These results underscore that pre-trained model selection plays a critical yet overlooked role in OOD generalization and calibration.

\subsection*{Contributions}
\label{sec:contribution}

% [Key findings]:  Contribution
This work highlights three key insights into model selection for OOD generalization and calibration: 

\begin{itemize}
      \item Larger model parameter size and bigger pre-training dataset improve OOD generalization performance (\cref{fig:all-pacs-avg_test_acc_pram_dataset}).
      \item Similarly, calibration issues are mitigated with larger models and datasets.
      This new evidence, comes to complete the previous, partial understanding that modern deep learning networks calibrate worse than \update{small and shallow models} (\cref{fig:all-pacs-avg_test_ece_pram_dataset}). 
      \item The generic model design and training strategy produces the most transferable pre-trained models, compared to techniques that overfit on ImageNet-1K (\cref{fig:all-in1k_acc-avg_test_acc} and \cref{fig:v7-num_params-avg_test_acc}). 
\end{itemize}


% We also observe the consistent trend of training strategies for downstream tasks and characterize correlation behavior depending on distributional shift datasets. 
Our systematic findings advocate an increased focus on pre-trained model selection. Specifically, we highlight best practices like using the largest pre-trained models and datasets and avoiding techniques tailored narrowly for in-distribution performance. These insights could redefine approaches to OOD generalization and calibration.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Preliminary}\label{sec:preliminary}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \item[Model Parameter Size and Dataset Size:]
% These dimensions significantly shape the effectiveness of fine-tuning. Generally, larger models and datasets yield superior results. However, extremely large models can pose challenges due to increased computational requirements and potential overfitting. The pre-trained models examined in our study are listed in Table \ref{ap:tab:all_models}.


Before delving into our experiments and findings, it is crucial to lay the groundwork by defining key concepts that underpin our research.

\begin{description}[leftmargin=*,itemsep=0pt,topsep=0pt]
    
\item[OOD Generalization:]
Out-of-distribution (OOD) generalization encompasses a range of concepts, including domain generalization, domain adaptation, robust generalization, and adversarial training. It aims to represent a model's capacity to accurately interpret and handle data that it has not encountered during training.
This aspect is crucial for ensuring that models perform effectively in real-world scenarios where data can vary from the training set distribution.

\item[Uncertainty Quantification:]
Quantifying the model prediction's uncertainty is vital for understanding the reliability of the model prediction. This becomes particularly relevant in high-stakes domains like cancer detection, where a model's overconfidence can have serious consequences.
\citet{guo2017calibration} showed that ``modern'' deep neural networks (in 2017), such as \modelname{ResNet-110}, tend to be overconfident in their predictions compared to classical neural networks such as \modelname{LeNet-5}, highlighting the need for reliable uncertainty quantification.

Expected Calibration Error (ECE) is a widely used metric for quantifying uncertainty. It measures the discrepancy between a model's predicted confidence and its actual accuracy. The formula is given as:
% 
\begin{align}
\mathrm{ECE}=\sum_{m=1}^{M} \frac{\left|B_{m}\right|}{n}\left|\operatorname{acc}\left(B_{m}\right)-\operatorname{conf}\left(B_{m}\right)\right|.
\end{align}
% 
Accuracy $\operatorname{acc}\left(B_{m}\right)$ and confidence $\operatorname{conf}\left(B_{m}\right)$ are defined as follows
% 
\begin{align}
\operatorname{acc}\left(B_{m}\right)=\frac{1}{\left|B_{m}\right|} \sum_{i \in B_{m}} \mathbf{1}\left(\hat{y}_{i}=y_{i}\right),\quad \operatorname{conf}\left(B_{m}\right)=\frac{1}{\left|B_{m}\right|} \sum_{i \in B_{m}} \hat{p}_{i},
\end{align}
% 
where $B_{m}$ is the set of samples whose prediction scores fall into bin $m$, $\hat{p_{i}}$ is the confidence of sample $i$, $y_{i}$ is the true label,  $\hat{y_{i}}$ is the predicted label, and $n$ is the total number of samples in all the bins.

While ECE provides a useful overall measure of calibration, it is important to interpret ECE carefully, especially when accuracy is low. Models that make random predictions or fail to learn can still achieve low ECE.
Therefore, when comparing models, it is critical to consider ECE primarily in high-accuracy regions. 
% Focusing on the ECE of well-performing models provides a more meaningful characterization of uncertainties for inputs the model can actually predict correctly. 

\end{description}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Works}\label{sec:relatedworks}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{description}[leftmargin=*,itemsep=0pt,topsep=0pt]
    
\item[OOD Generalization Algorithms and Benchmarks:]%\mbox{}\\
In recent years, various algorithms have been proposed to improve OOD generalization, such as invariant risk minimization~\citep{Arjovsky19}, group distributionally robust optimization~\citep{sagawa2019distributionally}, risk extrapolation~\citep{krueger2021out}, correlation alignment~\citep{sun2016deep}, gradient variances control~\citep{rame2022fishr}.
However, their performance depends heavily on the dataset characteristics, and no optimal algorithm has been identified. Furthermore, empirical risk minimization still achieves competitive performance on covariate shift~\citep{Ahuja20}.
DomainBed~\citep{Gulrajani21} has become a standard benchmark consisting of image classification datasets with different domain shifts for evaluating OOD generalization. Other benchmarks have also been introduced, such as WILDS ~\citep{koh2021wilds} for various data types and distributional shifts, WOODS~\citep{gagnon2022woods} focusing on time series data, and TableShift~\citep{gardner2023benchmarking} for tabular data.

\rev{
\item[Uncertainty Calibration Benchmark:]%\mbox{}\\
More recent studies have also evaluated modern architectures in comparison with calibration and robustness benchmarks, and \citet{minderer2021revisiting} argue, as do \citet{guo2017calibration}. that the ECE degrades with larger models.
There are four differences between their studies and ours.

First, our protocol targets pre-trained model selection for fine-tuning tasks, whereas their protocol targets scratch training.
Second, we evaluate in the context of OOD generalization, and they evaluate on robustness benchmarks such as image corruption and perturbation (We also provide the results in \cref{ap:fig:ood-imagenet-variants}, in addition to the OOD generalization benchmarks).
Third, we evaluate more than 100 models, including a wide range of architectures, training strategies, model parameter size, and training data, as well as an exhaustive hyperparameter search, which has been done with a limited number of model families and training sets (28 at most) in the previous study.
Finally, we conduct a systematic evaluation of the impact of the number of parameters in the pre-trained model and the size of the pre-training dataset on both OOD generalization and calibration metrics. This is an attempt to explore an aspect that has not been previously investigated.
}




\item[Pre-trained Model Selection for Downstream Tasks:]%\mbox{}\\
% Robustness measure 
Fine-tuning pre-trained models has become the prevalent approach for OOD generalization tasks~\citep{Gulrajani21}. However, most works have focused on advancing algorithms, with a limited investigation into pre-trained model selection.
Some analyses~\citep{goldblum2023battle, zhang2022delving, 10191806, yamada2022does, andreassen2021evolution} have compared model architectures on robustness benchmarks~\citep{hendrycks2021many,hendrycks2021natural,beyer2020we,recht2019imagenet, hendrycks2019robustness}. 

However, in studies that measured the effect of pre-trained model selection for OOD generalization, the number of pre-trained models for comparison is limited.
For example, \citet{carlucci2019domain} proposed pre-training \modelname{CNNs} to solve puzzles to learn features useful for domain generalization and evaluated them using ResNet18 and AlexNet as pre-trained models.
\citet{li2022sparse} proposed a \modelname{GMoE} model that replaces the FFN block of the \modelname{ViT} architecture with a mixture-of-experts block and compared it with the \modelname{CNN} and  \modelname{ResNet}.
\citet{zhang2023unified} have tested their proposed method on 12 pre-trained models (\modelname{CNN\nobreakdash-}, \modelname{MLP\nobreakdash-}, and \modelname{Transformer-based}) in the context of test time domain adaptation. Except for \modelname{ResNet}, there are no comparative experiments on more than three different parameter sizes or pre-training data in the same model architecture, and no analysis of parameter sizes or datasets was conducted. 
\citet{cha2022domain} and~\citet{arpit2022ensemble} conducted evaluation experiments using \modelname{RegNetY-16GF} as a pre-training model in addition to \modelname{ResNet} to evaluate the validity of their proposed method.

\rev{
\citet{yu2021empirical} focused on only \modelname{BiT}, \modelname{ViT}, and \modelname{ResNet} architecture, \citet{zhang2022delving} focused on only \modelname{ViT}, while \citet{vishniakov2023convnet} studied more in detail of \modelname{ViT} and \modelname{ConvNeXt} architecture in the context of downstream tasks.
}
In addition, all related works mentioned above pay no attention to ECE under distributional shift.

\item[Trend of Larger Models and Datasets:]%\mbox{}\\
Recent evidence~\citep{mikami2022scaling} suggests that larger models and bigger pre-training datasets lead to better generalization in downstream tasks of Syn2Real~\citep{yasarla2020syn2real}. 
Not only in downstream tasks, this trend is also observed in the context of scaling laws~\citep{kaplan2020scaling, zhai2022scaling, hestness2017deep}.
We systematically verify if this trend applies to OOD generalization and calibration scenarios.

\rev{
On another note, \citet{ruan2021optimal} has taken on the challenge of improving OOD generalization performance in multimodal models using CLIP \citep{clip_paper}. However, as shown by \citet{zhang2023unified}. they point out that the images such as LAION-2B\footnote{\url{https://laion.ai/blog/laion-5b/}} that CLIP has trained on contain images analogous to the sketch domain of DomainNet \citep{peng2019moment}, one of the evaluation datasets for OOD generalization. Since this could potentially undermine our problem setting for evaluating OOD generalization, although we have performed evaluation experiments on CLIP models as pre-trained models, we only present these settings and results in \cref{ap:clip,ap:additional_results_clip}.
}


\item[Link between OOD Generalization and Calibration:]%\mbox{}\\
Recent theoretical study~\citep{wald2021calibration} has shown that multi-domain calibration is equivalent to invariant risk minimization~\citep{Arjovsky19}, a popular OOD generalization technique. 
Some empirical observations indicate that techniques good at OOD generalization also achieve lower ECE~\citep{ovadia2019can, immer2021scalable, naganuma2023necessary, yoshida2024understanding}. 




We examine if this correlation holds for varying pre-trained models \rev{under distributional shift} as well.

\end{description}

% \subsection{Fine-Tuning Paradigm}
% The choice of source models for fine-tuning and transfer learning has been a subject of debate and exploration in the field of machine learning~\citep{kolesnikov2020big}. While earlier trends suggested that using VGG models pre-trained on ImageNet-1k was a popular choice due to its simplicity and versatility~\citep{too2019comparative, tammina2019transfer}, there seems to be a shift towards using other models. The DomainBed framework~\citep{Gulrajani21}, for instance, relies on the ResNet-50 model as a default choice for fine-tuning purposes, indicating a broader range of models being considered for fine-tuning.

% \subsection{Large-Scale Models and Datasets}
% In the context of model size, research indicates that increasing the scale of a model significantly improves its performance. This trend is evident in the large language model domain~\citep{kaplan2020scaling} and also in computer vision~\citep{zhai2022scaling}. There are studies that liken the role of larger models to ensembles due to the improved performance resulting from increased model size~\citep{abe2022deep}. Additionally, there has been work on analyzing how increasing the dataset size impacts model performance~\citep{hestness2017deep}.

% \subsection{OOD Generalization and Uncertainty}
% In the realm of  OOD generalization and uncertainty, comparisons between various proposed algorithms~\citep{Arjovsky19, sun2016deep, krueger2021out} have shown that substantial improvements can be made, excluding extreme cases like correlation shift~\citep{arjovsky2019invariant, ming2022impact}. This observation inspires us to reassess the choice of the pre-trained model used in the fine-tuning process.


% On the dataset comparison front, there are papers quantitatively comparing statistical information from various OOD datasets~\citep{ye2022ood}. Our study takes a more practical approach by focusing on diversity shifts.

% For model comparison, prior research suggests that Vision Transformers (ViT) are potentially more robust for OOD generalization~\citep{bhojanapalli2021understanding}. However, a detailed examination of their uncertainty in terms of ECE is still lacking. Moreover, there is a lack of comparison with other models like ConvNets, or with respect to the pre-training datasets used. 

On another note, our experiments adopted pre-trained models from the PyTorch Image Models library~\citep{rw2019timm}, also known as \texttt{timm}. It benchmarks models on ImageNet OOD test sets, such as ImageNet-R~\citep{hendrycks2021many}, ImageNet-A~\citep{hendrycks2021natural}, ImageNet-v2~\citep{recht2019imagenet}, and ImageNet-Real~\citep{beyer2020we} which is beneficial for our study.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experimental Setup}\label{sec:experiments}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[t]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{llrr}
    \toprule
         Dataset & Domains  & \#Images & \#Classes   \\
    \midrule
         PACS & \textbf{\texttt{art}}, \texttt{cartoon}, \texttt{photos}, \texttt{sketches}     & 9,991  &   7      \\
         
         OfficeHome & \textbf{\texttt{art}}, \texttt{clipart}, \texttt{product}, \texttt{real} & 15,588  &  65      \\
         
         DomainNet  & \shortstack{\textbf{\texttt{clipart}}, \texttt{infograph}, \texttt{painting}, \texttt{quickdraw}, \texttt{real}, \texttt{sketch}} & 586,575   & 345 \\
         
         VLCS       & \textbf{\texttt{VOC2007}}, \texttt{Caltech101}, \texttt{LabelMe}, \texttt{SUN09} &  10,729 & 5 \\
         
         Camelyon17       & \shortstack{\textbf{\texttt{Hospital1}}, \texttt{Hospital2}, \texttt{Hospital3},  \texttt{Hospital4}, \texttt{Hospital5}} &  455,954 & 2 \\
    \bottomrule
    \end{tabular}
    }
    \caption{Datasets from the DomainBed \citep{Gulrajani21} and WILDS \citep{koh2021wilds} Banckmark used in our experiments. Domains with bold faces are used as out-of-distribution test domains, and others are used for (in-domain) training and validation.}
    \label{tab:domainbed-workloads}
    \vspace{-3mm}
\end{table}


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/id_val_acc-ood_test_acc.pdf}
    \caption{The relationship between in-domain (ID) validation accuracy and out-of-distribution (OOD) test accuracy of all experiments. When ID validation accuracy is high enough, ID and OOD accuracy are highly correlated, the ``training-domain validation set'' scheme can select near-optimal models.}
    \label{fig:id_val_acc-ood_test_acc_pacs}
    \vspace{-4mm}
\end{figure}

Our experiments evaluate the OOD generalization accuracy (or error) and ECE of \update{100} pre-trained models fine-tuned on \update{five} OOD image classification datasets, namely PACS, OfficeHome, DomainNet, and VLCS, from the DomainBed benchmark~\citep{Gulrajani21}  (see also \cref{tab:domainbed-workloads}).
\update{
Additionally, we conducted medical image classification experiments using Camelyon17 datasets from WILDS benchmark~\citep{koh2021wilds} to cover other types of OOD generalization task evaluation (\cref{ap:results_camelyon}). 
}
% \rev{
% The experimental results from Camelyon17 dataset align with the trends observed in DomainBed. Details of the experiments and their outcomes are provided in \cref{ap:results_camelyon}
% }

Pre-trained models are selected from the \texttt{timm} library~\citep{rw2019timm}, which offers a vast collection of over a thousand pre-trained image classification models. 
Among them, we use models pre-trained on \update{families of} ImageNet to minimize data overlap with the DomainBed and WILDS datasets, since our interest lies in OOD generalization.
Specifically, we adopt pre-training datasets of ImageNet-1k (1k categories, 1.4M images), ImageNet-12k (12k categories, 12M images), ImageNet-21k (21k categories, 14M images), and ImageNet-22k (22k categories, 14M images).
While \texttt{timm} also offers models pre-trained on larger datasets, such as LAION~\citep{schuhmann2022laionb} consisting of billions of images, we refrain from utilizing them due to their excessive size, which raises concerns about the potential inclusion of OOD test data.
\rev{In addition to the models pre-trained on image data only, we validate CLIP models, which are pre-trained on image-text pairs (\cref{ap:clip}).}
Selected \update{100} pre-trained models, varying parameter sizes from 3M to 600M, are listed in \cref{ap:tab:all_models}.
Further details are explained in \cref{ap:all_models}.

For fine-tuning, we follow DomainBed's experimental protocol.
The key difference from the original protocol is that we use various pre-trained models from \texttt{timm}, rather than fixing the pre-trained model only to \modelname{ResNet-50}.
To prioritize the exploration of models under fixed computational constraints, we adopt a simple evaluation approach different from the original DomainBed.
Namely, we select each dataset's first domain listed in \cref{tab:domainbed-workloads} as the OOD test domain and use the remaining domains as (in-domain) training and validation data.


Another difference from DomainBed is the choice of optimizer for fine-tuning.
We adopt SGD with a momentum of 0.9 as a default optimizer rather than Adam~\citep{Kingma15}, as SGD with Momentum is more effective in OOD generalization~\citep{naganuma2023empirical} (we confirm this in \cref{fig:optim_lr_val_acc,fig:optim_lr_test_acc}).
In addition, we fine-tune models with adaptive optimizers when they are used for pre-training: RMSProp for \modelname{EfficientNets}, AdamW for \modelname{ConvNeXts}, and Adam for \modelname{ViTs}.

Their hyperparameters, learning rates, and weight decay rates are selected using in-domain validation data, as we cannot access OOD data.
This selection is referred to as the ``training-domain validation set'' scheme in the DomainBed benchmark~\citep{Gulrajani21} and is capable of finding near-optimal models when in-domain validation accuracy is high enough (\cref{fig:id_val_acc-ood_test_acc_pacs}).
Further details on hyperparameter selection are described in \cref{ap:hyperparamters}.
We also run experiments over three different random seeds, and their effects on the final results are negligible, as shown in \cref{ap:tab:mean_std}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Results}\label{sec:results}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In the remaining text, we report OOD generalization performance and ECE on the held-out test domain data of models selected by the above-mentioned validation scheme.
Full results and a detailed analysis for each model architecture are shown in \cref{ap:full_results} and \cref{ap:results_per_model}.

\begin{figure}[t]
    \centering	
    \includegraphics[width=\linewidth]{figs/all-pacs-avg_test_acc_ece_pram_dataset.pdf}
\caption{
(a,b) OOD test error rates (lower is better) with respect to the number of parameters (a, log-scale) and the pre-training dataset sizes (b) on the PACS dataset. In the right panel, the same model architectures with different pre-training datasets are connected by dashed lines. We can observe that \textbf{the number of parameters and the pre-training dataset sizes contribute to the OOD generalization}. Presented models are selected for a better view. Results of other OOD datasets with all models are presented in \cref{ap:fig:all-test-acc-test-ece,ap:fig:all-all-test-acc-test-ece,ap:fig:dataset-avg_test_acc-avg_test_ece}. 
(c,d) OOD expected calibration error (lower is better) with respect to the number of parameters (c) and the pre-training dataset sizes (d) on the PACS dataset. In the right panel, the same model architectures with different pre-training datasets are connected by dashed lines. We can see trends that \textbf{the number of parameters and the pre-training dataset sizes improve ECE}. Presented models are selected for the better view. Results of other OOD datasets with all models are presented in \cref{ap:fig:all-test-acc-test-ece,ap:fig:all-all-test-acc-test-ece,ap:fig:dataset-avg_test_acc-avg_test_ece}.
}
\label{fig:all-pacs-avg_test_acc_pram_dataset}
\label{fig:all-pacs-avg_test_ece_pram_dataset}
\vspace{-4mm}
\end{figure}    


\subsection{Scaling Trend: OOD Generalization}\label{sec:scaling_ood_generalization}

Our comprehensive experiments reveal several consistent and significant trends in how pre-trained model selection impacts out-of-distribution generalization performance.

First, we find that increasing the number of parameters in pre-trained models leads to noticeable gains in OOD accuracy across almost all model architectures examined, as shown in \cref{fig:all-pacs-avg_test_acc_pram_dataset}. Similarly, pre-trained models on larger dataset sizes yield substantial OOD performance improvements. These trends hold not just for the PACS examples shown here but also generalize to other evaluation datasets for domain generalization (\cref{ap:fig:all-all-test-acc-test-ece,ap:fig:dataset-avg_test_acc-avg_test_ece}).
Second, when comparing models with similar parameter sizes, we observe that \modelname{ViT} and \modelname{ConvNeXt} architectures tend to achieve higher OOD accuracy than conventional \modelname{CNN} architectures like \modelname{ResNet} and \modelname{EfficientNet}. This suggests the benefits of more recent model architectures specialized for computer vision tasks.

As a remarkable observation, we also find that OOD error decreases almost linearly on a log-scale of parameters as the pre-trained model size increases \rev{as shown in \cref{fig:all-pacs-avg_test_acc_pram_dataset}~(a)}. This implies the \textbf{sign of scaling laws} and hints at shared underlying mechanics that drive performance gains in downstream domain generalization tasks.
Lastly, through targeted experiments on \modelname{ConvNeXt} and \modelname{ViT} models, we verify that increasing the pre-training dataset size significantly boosts OOD accuracy. This further underscores the importance of large-scale pre-training data for enhancing OOD generalization.

In summary, our extensive empirical results reveal consistent trends that bigger pre-trained model sizes and larger pre-training datasets lead to substantial and reliable improvements in out-of-distribution generalization performance across diverse model architectures and evaluation datasets. These insights provide practical guidance for pre-trained model selection when targeting OOD tasks.


% \begin{figure}[t]
%     \centering	
%     \includegraphics[width=\linewidth]{figs/all-pacs-avg_test_acc_ece_pram_dataset.pdf}
% \caption{OOD test error rates (lower is better) with respect to the number of parameters (left, log-scale) and the pre-training dataset sizes (right) on the PACS dataset. In the right panel, the same model architectures with different pre-training datasets are connected by dashed lines. We can observe that \textbf{the number of parameters and the pre-training dataset sizes contribute to the OOD generalization}. Presented models are selected for the better view. Results of other OOD datasets with all models are presented in \cref{ap:fig:all-test-acc-test-ece,ap:fig:all-all-test-acc-test-ece,ap:fig:dataset-avg_test_acc-avg_test_ece}.}
% \label{fig:all-pacs-avg_test_acc_pram_dataset}
% \end{figure}    



\subsection{Scaling Trend: Uncertainty Calibration}\label{sec:scaling_calibration}
Our experiments reveal interesting insights into how pre-trained model selection affects uncertainty calibration performance as quantified by ECE, as depicted in \cref{fig:all-pacs-avg_test_ece_pram_dataset}~(b).
First, we find that increasing the number of parameters in pre-trained models leads to lower ECE, mirroring the trends observed for OOD generalization. Using pre-trained models trained on larger dataset sizes also improves calibration.

These results contrast with prior work that found modern deep networks like \modelname{ResNet-110} to have significantly higher ECE than small networks like \modelname{LeNet-5}, despite their greater accuracy \citep{guo2017calibration, minderer2021revisiting}. Surprisingly, we demonstrate that at even larger parameter scales beyond \modelname{ResNet-110}, the trend reverses, and ECE starts to decrease with model parameter size.
Specifically, ECE reduces almost linearly as pre-trained model size increases on a log scale, analogous to the scaling laws for OOD error. This suggests there may be shared principles governing calibration improvements in downstream tasks.

\rev{In summary, increasing the size of the pre-trained model and pre-training data boosts OOD generalization and leads to more reliable uncertainty estimates as measured by ECE}. Our results overturn prior observations that modern deep networks suffer from higher ECE and underscore the potential of large-scale pre-trained models to address calibration challenges.

% \begin{figure}[t]
%     \centering	
%     \includegraphics[width=0.5\linewidth]{figs/all-pacs-avg_test_ece_pram_dataset.pdf}
% \caption{OOD expected calibration error (lower is better) with respect to the number of parameters (left) and the pre-training dataset sizes (right) on the PACS dataset. In the right panel, the same model architectures with different pre-training datasets are connected by dashed lines. We can see trends that \textbf{the number of parameters and the pre-training dataset sizes improve ECE}. Presented models are selected for the better view. Results of other OOD datasets with all models are presented in \cref{ap:fig:all-test-acc-test-ece,ap:fig:all-all-test-acc-test-ece,ap:fig:dataset-avg_test_acc-avg_test_ece}.}
% \label{fig:all-pacs-avg_test_ece_pram_dataset}
% \end{figure}

\subsection{Pre-trained Models can Overfit to Training Set}\label{sec:overfit_imagenet}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/all-in1k_acc-avg_test_acc.pdf}
    \caption{Correlation between ImageNet-1k validation accuracy and out-of-distribution test accuracy. OOD test accuracy shows a strong positive correlation with ImageNet-1k validation accuracy. However, \modelname{EfficientNets} fall below the trend of other models, suggesting that \emph{they may be overfitting to ImageNet-1k.}}
    \label{fig:all-in1k_acc-avg_test_acc}
\end{figure*}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/v7-num_params-avg_test_acc.pdf}
    \caption{Out-of-distribution test accuracy of \modelname{ResNets}~\citep{he2016deep} with different training schemes. The results of the original \modelname{ResNets} are connected by dashed lines. Although extensive training recipes~\citep{wightman2021resnet} improve ImageNet-1k performance, their fine-tuned OOD results often underperform the original ones.}
    \label{fig:v7-num_params-avg_test_acc}
    \vspace{-4mm}
\end{figure}


\rev{We observe that some pre-trained models are likely to overfit to training set such as ImageNet-1k.}
\Cref{fig:all-in1k_acc-avg_test_acc} presents the relationship between ImageNet-1k validation accuracy and OOD test accuracy.
As can be seen, the \modelname{EfficientNet} models tend to fall below the trendlines of other models, suggesting that they are more prone to overfitting to ImageNet-1k and do not transfer well to OOD datasets. 
This overfit could be attributed to \modelname{EfficientNets} being designed by neural architecture search~\citep{tan2019efficientnet}, where the components of networks are searched to maximize validation performance.
Although improvement of pre-training methods, such as using extensive data augmentation~\citep{cubuk2019autoaugment,xie2020adversarial}, enhances OOD generalization performance (\cref{fig:v6-num_params-avg_test_acc}), overfit trends unchanged as evident in \cref{ap:fig:all-all-in1k-test-acc-test-ece}.
This figure also depicts that fine-tuned EfficientNets degenerates calibration on the OOD datasets.
In contrast, \modelname{RegNets}~\citep{radosavovic2020designing} seems to avoid overfitting, probably because they are optimized at a meta-level (design principles), not at a component level.

\citet{wightman2021resnet} reported that \modelname{ResNet-50} with renewed training recipes, including additional data augmentation and longer training, attains more than 5\% ImageNet-1k accuracy improvement over the original setting.
\Cref{fig:v7-num_params-avg_test_acc} displays the comparison of the \modelname{ResNets} pre-trained with the original and the updated recipes: a new training recipe introduced in \texttt{torchvision}\footnote{Details are described in \url{https://pytorch.org/blog/how-to-train-state-of-the-art-models-using-torchvision-latest-primitives}.} referred to as \modelname{v2} and others proposed in~\citep{wightman2021resnet} referred to as \modelname{A1}-\modelname{A3}.
Although models trained with these new training recipes improve ImageNet-1k performance, \modelname{A1}-\modelname{A3} often perform inferior to the original ones under the same fine-tuning setting.
Contrarily, the \modelname{v2} models consistently outperform the original models.
These results may indicate that certain aspects of pre-training strategies in \citet{wightman2021resnet} may lead to overfitting to ImageNet-1k.
Disentangling the specific factors causing the OOD performance degeneration is challenging, due to the various techniques employed in these recipes.
However, it is possible to guess that binary cross-entropy loss and/or Adam optimizer during pre-training are attributed to the issue.
It is also worth noting that extensive data augmentation, such as RandAugment~\citep{cubuk2020randaugment} and AugMix~\citep{hendrycks2020augmix}, improves the OOD generalization as in \cref{ap:fig:v7-r50-in1k_acc-avg_test_acc}.

These overfit phenomena of \modelname{EfficientNets} and enhanced \modelname{ResNets} cannot be observed on ImageNet OOD test sets, such as ImageNet-A, as presented in \cref{ap:fig:all-imagenet1k-imagenet-variants}.
Rather, \modelname{EfficientNets} and \modelname{ResNets} with \modelname{A1-A3} recipes are aligned with the correlations between the performance of ImageNet-1k and ImageNet OOD test sets.
These findings suggest that the generalization on pre-training datasets, such as ImageNet-1k, does not directly translate to the generalization after fine-tuning.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Other Findings}\label{sec:other_findings}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Above three are the major findings, but other findings of this study are briefly described. 
Details are given in \cref{ap:findings}.
First, in the pre-training phase, supervised pre-training with AugReg as a data augmentation approach improves OOD test accuracy compared to self-supervised methods like DINO and MAE. 
Second, as prior work \citep{naganuma2023empirical} suggests advantages for SGD with momentum over adaptive optimizers for OOD generalization, this study confirmed SGD with momentum consistently outperforms other optimizers when fine-tuning diverse architectures, including \modelname{ViT} and \modelname{EfficientNet.}
Third, the impact of weight decay on OOD performance varies across datasets. While stronger regularization improves calibration, it can hinder OOD accuracy on datasets with visually distinct domains, as shown in \cref{fig:wd-num_params-avg_test_acc}. 
The ablation studies for sensitivity and seed of hyperparameters are shown in \cref{ap:ablation_study}.
% }

\rev{
Analysis of ImageNet variant datasets for robustness benchmarks suggests a positive correlation between model robustness on ImageNet variants and domain generalization performance, with improvements on sampling bias datasets showing a stronger correlation compared to robustness benchmarks as shown in \ref{ap:fig:ood-imagenet-variants}.

Additionally, \cref{ap:results_camelyon} shows the results evaluated on the Camelyon17 datasets, aligning with the trends observed in DomainBed.
\Cref{ap:additional_results_clip} shows the results of CLIP models, which align with other models in terms of test accuracy.
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Discussion and Conclusion}
\label{sec:conclusion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \TODO{better guidance / guiding future research / our result is collective despite that a lot of work is working on fancy methodology / pre-trained model selection is more powerful than that we thought}


% In this work, \update{we have systematically and extensively} evaluated the effect of pre-trained model selection on out-of-distribution generalization and uncertainty calibration.

\update{
Our results are useful to practitioners due to their prescriptive nature:
our systematic study on over 100 pre-trained models yielded that in the OOD setting with pretraining, larger architectures using larger training sets achieve better out-of-distribution generalization and calibration.
We also found that non-generic training strategies---for example, the ones specifically designed to maximize in-distribution performance for ImageNet-1k on smaller models---do not achieve good OOD performance, indicating overfitting to the pre-training dataset.

% Our contributions are to guide future direction as a collective study, a systematic and extensive evaluation of pre-trained model selection that contributes significantly to baseline improvement rather than fancy methodologies, 
% and to provide prescriptions for pre-trained model selection when considering OOD generalization and calibration.
}

% The experiments over \update{100} pre-trained models revealed that large-scale models and pre-training datasets drastically improve out-of-distribution generalization and calibration.
% We also found that some successful strategies on ImageNet-1k for smaller models do not translate well to OOD performance, indicating overfitting to pre-training datasets.

In light of these results, we summarize our findings as the following guidelines on pre-trained model selection for practitioners:
\begin{enumerate}
    \item Use large pre-trained models,
    \item Use models pre-trained on large datasets,
    \item Use models pre-trained using generic methodology (i.e.\ not specifically designed to maximize in-distribution performace on a specific architecture).
\end{enumerate}
Following these guidelines can substantially improve OOD generalization and calibration capabilities.

\update{
Our results can also prove to be useful to researchers, as they provide guidance for future work in the area. 
In particular, one important by-product of our results is a newfound appreciation of model selection as a strong baseline. This point is important because recent work providing new, complex methodology, yields results that are inferior to the ones we provide here based on simple model selection.
Future work on computation-efficient methods for the OOD setting is critical; we hope that our results will help researchers build those new, efficient methods on top of solid baselines.
}



% At the same time, the computational demands of large-scale models cannot be overlooked in applications requiring real-time responses. 
% Therefore, developing algorithms for OOD generalization and calibration for smaller models remains essential, which would also contribute to understanding the underlying mechanisms.
% Furthermore, investigating ``transfer-aware'' pre-training strategies holds promise, as the experiments demonstrated that smaller models pre-trained with good policies translate their ImageNet-1k capabilities to OOD environments.
% We hope our empirical findings and guidelines help steer future work on pre-trained model selection for out-of-distribution tasks.





% \begin{description}[leftmargin=*,parsep=0pt,topsep=0pt]
    
% \item[Discussion:]
% While our study focuses on models that fit within the capacity of a single GPU, the broader question of memorization versus generalization becomes even more significant in the context of larger models. How to discern whether a model is generalizing or simply memorizing data poses an intriguing challenge for future exploration and indicates the need to redefine what out-of-distribution generalization means in the realm of large models.

% \item[Conclusion:]
% Our study highlights the superior OOD performance of larger models, corroborating previous findings~\citep{bhojanapalli2021understanding}.
% In light of our results, we advocate for the use of state-of-the-art models rather than persisting with older ones, given the substantial improvements they can bring to out-of-distribution generalization capabilities. 
% However, we emphasize that the development of algorithms for OOD generalization remains crucial in understanding these mechanisms.

% \item[Future Work:]
% A promising avenue for future research would be to propose a benchmark or guideline indicating the optimal choice of a pre-trained model for a given downstream task. We conjecture that improvements in OOD performance relative to an increase in the number of parameters may reach a saturation point. Establishing a predictive curve fitting for this phenomenon could provide valuable insights for the selection of optimal models.

% \item[Limitations:]
% Several limitations to our study warrant mention. First, the number of validation datasets for downstream tasks was not extensive, potentially restricting the generalizability of our findings. Second, we have not fully explored the influence of algorithm selection --- our experiments were primarily conducted with Empirical Risk Minimization (ERM). Lastly, optimal tuning of hyperparameters such as batch size and optimizer selection remains an area that requires further investigation.
% \end{description}




==> section/broader_impact.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Broader Impact}\label{ap:impact}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This research aims to reveal the effect of model selection of the OOD generalization and calibration of deep learning models by systematic investigation. 
While this research has the potential to lead to more robust and reliable AI systems, it also presents potential for negative societal impacts.

On the positive side, this research can contribute to developing more robust and reliable AI systems that generalize well to real-world scenarios. This is crucial for applications such as medical imaging and autonomous driving, where the data encountered in real-world situations might differ from the training data. Additionally, the study's findings on uncertainty calibration can lead to more reliable AI systems that are better at understanding their own limitations, which is essential for high-stakes applications like medical diagnosis and financial risk assessment.

Our findings also provide concrete guidelines for pre-trained model selection, helping practitioners make informed decisions about which pre-trained models to use for their specific applications. Our systematic study on over 100 pre-trained models reveals that larger architectures trained on larger datasets consistently achieve better out-of-distribution generalization and calibration. This insight can streamline the model selection process and lead to more efficient development of robust AI systems. We also found that non-generic training strategies designed to maximize in-distribution performance on smaller models often fail to generalize well to OOD scenarios. This highlights the importance of using generic training methods that promote better transferability.

Beyond practical implications, this research can guide future research in the field. Our results demonstrate that model selection serves as a strong baseline, challenging the notion that complex new methodologies are always superior. This newfound appreciation for model selection can encourage researchers to build new, computation-efficient methods for OOD settings on top of solid, well-established baselines.

However, there are also potential negative societal impacts associated with this research. The study's focus on improving AI robustness and reliability could be misused to generate more convincing deepfakes or other forms of synthetic media for disinformation purposes. 

To mitigate these negative impacts, it is crucial to promote ethical guidelines and responsible use of this technology in research and development. Transparency is also essential, which can be achieved by thoroughly documenting the pre-training datasets and training procedures used for the models. 
This allows users to understand potential biases in the models and can help identify potential negative impacts and develop mitigation strategies for the responsible deployment of AI systems.

Overall, this research presents a valuable contribution to AI, especially computer vision, but it is crucial to carefully consider its broader impacts and implement mitigation strategies to ensure the responsible and ethical use of the technology.

==> section/checklist.tex <==

\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We describe contributions in the introduction and conclusion and also explain how to deliver this contribution in the main body of this paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We describe the limitation of our work in conclusion and discussion section (See \cref{sec:conclusion}).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our work is pure empirical work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We put the link\footnote{\url{https://anonymous.4open.science/r/Timm_OOD_Calibration-E828/README.md}} to our code in the appendix and describe all the detailed experimental protocols in \cref{ap:settings}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We put the link to our code in the appendix with README documents (See \cref{ap:settings}).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: A experimental setting is described in \cref{sec:experiments} and \cref{ap:settings} for more in detail.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We are conducting an ablation study in \cref{ap:ablation_study} on seed differences and sensitivity of hyperparameters. As a result, we have confirmed that the variance of accuracy in seed is sufficiently small in our experimental scope, and that the influence of model selection is much larger than that.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We described that information in \cref{ap:settings}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We follow the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We describe the positive and negative aspect of this work in \cref{ap:impact}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our scope does not include such a high-risk model.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have checked the license of datasets and models subjected to our study. Also, we described that information in \cref{ap:settings}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We only use public datasets/models and did not provide new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We did not do crowdsourcing experiments or research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: We only use public image datasets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}
